Goal-directed Generation of Discrete Structures with Conditional Generative Models

Despite recent advances, goal-directed generation of structured discrete data remains challenging. For problems such as program synthesis (generating source code) and materials design (generating molecules), finding examples which satisfy desired constraints or exhibit desired properties is difficult. In practice, expensive heuristic search or reinforcement learning algorithms are often employed. In this paper we investigate the use of conditional generative models which directly attack this inverse problem, by modeling the distribution of discrete structures given properties of interest. Unfortunately, maximum likelihood training of such models often fails with the samples from the generative model inadequately respecting the input properties. To address this, we introduce a novel approach to directly optimize a reinforcement learning objective, maximizing an expected reward. We avoid high-variance score-function estimators that would otherwise be required by sampling from an approximation to the normalized rewards, allowing simple Monte Carlo estimation of model gradients. We test our methodology on two tasks: generating molecules with user-defined properties and identifying short python expressions which evaluate to a given target value. In both cases, we find improvements over maximum likelihood estimation and other baselines.

==> content/background.tex <==
\section{Background}
\subsection{Sequence generation}
Sequence models are normally trained to maximize the log-likelihood of the data. It %processes real data sequences one step at a time and  
tries to be good at greedy predicting the next element of the sequence based on all previous elements \citep{graves2013generating}. The probability distributions of the sequence data is given by $p(\bx_{1\dots T}) = \prod_{t=1}^{T} p(\bx_t| \bx_{1\dots t-1})$ where each term $p(\bx_t|\bx_{1\dots  t-1})$ is modeled as a parametric function by using RNN. Once trained, one can generate the entire sequence by sampling from or taking the argmax of each individual term, i.e., $\bx_t = \argmax  p(\bx| \bx_{1\dots t-1})$.  To generate sequence with specific user desired properties, instead of modeling $p(\bx_{1\dots T})$, one could learn the conditional distribution $p(\bx_{1\dots T}|\by)$ where $\by$ is some property vector that we want our sequence to be conditioned on. This distribution follows similar  factorization, i.e., $p(\bx_{1\dots T}|\by) = \prod_{t=1}^{T} p(\bx_t| \bx_{1\dots t-1},\by)$ and can be trained by maximizing the conditional log likelihood, $\log p_{\theta}(\bx|\by) $, in a supervised manner.

\subsection{Maximum likelihood training}
Standard ML objective, in our case conditional log-likelihood, does not require any sampling or inference during training. This computational efficiency makes it an ideal candidate for sequence models. Neural sequence models \citep{bahdanau2014neural} \citep{sutskever2014sequence} have shown great potential in machine translation and speech recognition. However, the log-likelihood objective is only measured on the ground truth input-output pairs. The model is pushed to learn a distribution $p(\bx|\by)$ such that it is peaked at the corresponding ground truth $\bx$ for a given properties vector $\by$. Such an objective is originally designed for supervised prediction tasks where all we want is to match the input to the target output. However, for the conditional generation task, what we care about is to optimize the task reward, i.e., generate diver sequences that have properties as close as to the target.  ML training does not take into account the fact that for target properties, there exist other sequences that are different from the ground truth but still are acceptable. To account for such a disadvantage, few approaches emerged where mostly some level of data perturbation is applied. For example, the  RAML \citep{norouzi2016reward} proposed to add reward-aware perturbation to the target, \citet{xie2017data} applied data noising in the language model. Even though those works have shown improvement over the pure ML training, they make an implicit assumption that the underlying sequences are stable to small perturbation. This restricts the applicability of such models on other types of sequences than text. 



\subsection{Reinforce}
On the other hand, reinforcement learning directly optimizes the task reward, i.e., minimize the distance between the generated sequences property to the target property,  instead of using conditional log-likelihood as a surrogate.  By making use of external feedback function $R(\bx, \by)$, which is normally non- differentiable, one can evaluate and assign a reward to all the possible sequences. The model takes in to account all possible sequences that are proposed by the model and allocates probability mass according to the reward instead of trying to learn a point mass at the ground truth only. It learns a distribution $p_{\theta}(\bx|\by)$ from which you can get samples that have a high reward by maximizing expected reward $\mE_{p_{\theta}(\bx|\by)}R(\bx, \by)$. 
\citet{ranzato2015sequence} has shown the potential to REINFORCE over ML  objective in sequence generation tasks. The expected reward is often optimized using policy gradient estimator\citep{sutton2000policy} \citep{williams1992simple}. 


However, such an estimator involves a score function trick where the gradient is approximated by the reward weighted gradient of the log-likelihood of the proposed sequences from the model. Since the sequences that are proposed by the model also used as the target of the model and the reward is sparse, at the starting, such gradient approximation is quite noisy which makes training slow and inefficient.
Most often such estimator requires the incorporation of complicated additional variance reduction techniques to reach a descent convergence with an affordable computational and time cost. 
Control variate is one of the most commonly used variance reduction techniques which uses "baselines" \cite{greensmith2004variance}, to help reduce the variance without introducing bias, for example, the moving-average baseline \cite{williams1992simple}.
 Many efforts have been made to design proper baselines that are effective \cite{wu2018variance}. Besides subtracting baselines, other techniques such using a pre-trained model (trained with maximum log-likelihood objective) to warm start the training,  incorporating beam search or replay buffer during training are also frequently applied \citet{wiseman2016sequence,bunel2018leveraging}. \citet{sehnke2010parameter} proposed a novel policy gradient method called policy gradients with parameter-based exploration(PGPE) which uses an initial policy that is drawn from a  prior probability distribution,  and  then actions  are chosen deterministically. 
More recent works also focused on replacing the sampling distribution with some other more complex distribution which takes into account both the model and reward distribution \cite{ding2017cold}. However, all of the works require extra expensive search, optimization or complex sampling process which makes the training quite expensive both in terms of time and resources. Therefore in this work, we try to develop an easy alternative to optimize the expected reward. 


 


==> content/expressions.tex <==
% !TEX root =  ../aistats_main.tex

The synthetic data used in the expressions / ``calculator'' example is comprised of integer arithmetic expressions in python3.
The expressions used as training data are sampled randomly from the PCFG defined as:
{\scriptsize
\begin{verbatim}
  S ->  Expr Op Expr [1.0]
  Expr -> Number [0.4] | L Action R [0.2] | Action [0.4]
  Action -> Expr Op Expr [1.0]
  Number -> Nonzero Digits [0.9] | Nonzero [0.1]
  Nonzero -> 1 [0.1111] | 2 [0.1111] | 3 [0.1111] | 4 [0.1111] | 
             5 [0.1111] | 6 [0.1111] | 7 [0.1111] | 8 [0.1111] | 
             9 [0.1111]
  Digits -> Digit [0.95] | Digit Digits [0.05]
  Digit -> 0 [.1] | Nonzero [0.9]
  Op -> '+' [0.3] | '-' [0.3] | '*' [0.2] | '//' [0.2]
  L -> '(' [1.0]
  R -> ')' [1.0]
\end{verbatim}}
with the additional constraints expression that the value $y$ obtained by calling python \textsc{Eval} satisfies $-1000 < y < 1000$, 
and that the expression itself is at most 30 characters.
We generate 500,000 samples in this manner, which we then filter to remove duplicates, leaving a total of 308,772 unique (expression, value) pairs; 20,000 are set aside as a validation set.

In learning the conditional generative model $p_\theta(\bx | y)$, we rescale the input value $y$ by a factor of 1000, to ensure the input to the LSTM is in the interval $(-1, 1)$.
When sampling from $\bar R(\bx | y)$, a candidate $\bx$ is obtained by first sampling $y'$ from $\mathcal{N}(y' | y, 1)$, rounding the sampled $y'$ and truncating to $(-999, 999)$, and then uniformly sampling $\bx$ from all training examples such that \textsc{Eval}$(\bx) = \mathrm{round}(y')$.

==> content/literature_review.tex <==
% !TEX root =  ../main.tex

\section{Related work}
Many proposals for conditional generation of discrete structures are two-stage.
For example, focusing on molecule generation tasks, \citet{segler2017generating} train a RNN model on a large dataset of drug-like molecules; the RNN can then be used to generate a large body of candidate structures. These can later be screened post-hoc, though this can become unfeasible for rare properties, or uncommon combinations of multiple properties; this can be addressed by fine-tuning the network to produce molecules which more and more closely match a desired target. 
An alternative approach is to sidestep the discrete nature of the data entirely by applying latent variable models which map the discrete data to a continuous space. The learned continuous latent representation is then used in optimization to find sequences with the desired properties \citep{DBLP:journals/corr/Gomez-Bombarelli16,kusner2017grammar,dai2018syntax}.
However, these latent variable models, if no further restriction is applied, tend to perform poorly when compared to simpler sequence models in terms of  validity of generated sequences, and in terms of matching distributional statistics of the training data \citep{liu2018constrained,brown2019guacamol}.
Furthermore, these do not offer a direct approach to conditional generation --- either the generative model must be fine-tuned, or an additional (potentially expensive) optimization algorithm must be run using the continuous latent space.

A recent exception is \citet{DBLP:journals/corr/abs-1811-09766} which learns an autoencoder where the decoder takes the latent code and the desired property as an input. 
A mutual information term is used in training to steer the model towards generating molecules whose target properties match the input value.  Similar work appeared in conditional text generation \cite{hu2017toward}, where a constraint is added so
that the generated text matches a target property by jointly training a VAE with a discriminator using a wake-sleep algorithm; the model, though generic, has only been used with binary properties.
In both cases, only conditioning on a single scalar property is considered, whereas in real-world goal-directed generation problems there may be many simultaeneous properties of interest.

%
%Latent variable models such as 
%\citet{DBLP:journals/corr/Gomez-Bombarelli16, kusner2017grammar, jin2018junction}
%applied variational autoencoders either on string-based or graph-based representation of molecules. 
%However, these do not perform direct conditional generation, they are trained in an \textit{unsupervised} manner, agnostic to any property which later may need to be optimized. 
%A recent exception is \citet{DBLP:journals/corr/abs-1811-09766} which learns an autoencoder where the decoder takes the latent code and the desired property as an input. 


%hybird models
\citet{Guimaraes2017-az, De_Cao2018-iz,you2018graph} propose to use hybrid models that combine adversarial training with reinforcement learning objectives.
% This takes the generation task one step closer towards conditional generation, where the generated molecules properties are optimized towards a certain goal. 
The goal is only defined as generating sequences that some certain property is enhanced. 
Thus each time to condition the generation with a certain value of the property, the model needs retraining.
Such models still have no total control on the property of the molecules that are being generated. 

%Along the line of ML training
Latent variable models even though can generate continuous representations of the discrete structures, which then can be used to search for the sequence with the target property, suffers from low validity performance if no further restriction is applied \citep{dai2018syntax,liu2018constrained}. 
In contrast, the sequence-based models such as the afore-mentioned \citet{segler2017generating} perform well in terms of validity, although they also require fine-tuning afterward to redirect generation towards the goal.
%\citet{segler2017generating} applied RNN type models to generate sequences unconditionally. Such models require fine-tuning afterward to redirect the generation towards the goal. 


Most of the existing work for conditional generation, such as program synthesis, machine translations and structure output prediction adopt a sequence generation paradigm similar to neural machine translation, in which sequence-to-sequence models are trained to maximize the likelihood of known reference programs \citep{bahdanau2014neural, sutskever2014sequence}
However, for the conditional generation task, what we care about is to optimize the task reward, i.e., generating sequences that have properties as close as possible to the target.  
ML training does not take into account the fact that for a target property, there exist many candidates that are different than the ground truth but still acceptable. 
To account for such a disadvantage, a few approaches have emerged where some level of data perturbation is applied. 
For example, reward-augmented maximum likelihood (RAML) proposed in \citet{norouzi2016reward} adds reward-aware perturbations to the target, and \citet{xie2017data} applied data noising in language models. 
Even though those works have shown improvement over the pure ML training, they make an implicit assumption that the underlying sequences' properties are relatively stable with respect to small perturbation. This restricts the applicability of such models on other types of sequences than text. 

Instead of using conditional log-likelihood as a surrogate, direct optimization of task reward has been considered as a best practice for goal-oriented sequence generation tasks. Various RL approaches have been applied for sequence generation, such as policy gradient \cite{ranzato2015sequence}
and actor-critic \cite{bahdanau2016actor}. However, maximizing the expected reward is costly, sometime even intractable. Most often it requires incorporation of complicated additional techniques to reach a descent convergence with an affordable computational and time cost. Many works have been developed around for reducing the variance of such gradient estimator, such as applying various variance reduction techniques \cite{greensmith2004variance}, warm starting from a pre-trained model, incorporating beam search \citet{wiseman2016sequence,bunel2018leveraging} or replay buffer during training. 
 More recent works also focused replacing the sampling distribution with some other complicated distribution which takes into account both the model and reward distribution \cite{ding2017cold}. However, those techniques are still expensive and hard to train. Therefore in this work we try to develop an easy alternative to optimize the expected reward.


%%% MOVED THE FOLLOWING TO BEGINNING OF METHOD SECTION INSTEAD:
%Considering the limitations of the work discussed above,
%in this paper, we try to tackle conditional generation in one step, training a model which requires no further optimization and gives us total control on the generated sequences properties. 
%To avoid the limitations of ML training, we start with an RL objective.
%We sidestep the high variance of the gradient estimation issue which would be in part if we directly apply policy gradient, by developing its equivalent where we do not need to sample from the model and search for direction with high reward. Instead, we sample from approximated normalized reward distribution which directly puts us in the right direction during optimization.


% 
